BotBuster: Multi-platform Bot Detection Using A Mixture of Experts

Despite rapid development, current bot detection models still face challenges in dealing with incomplete data and cross-platform applications. In this paper, we propose BotBuster, a social bot detector built with the concept of a mixture of experts approach. Each expert is trained to analyze a portion of account information, e.g. username, and are combined to estimate the probability that the account is a bot. Experiments on 10 Twitter datasets show that BotBuster outperforms popular bot-detection baselines (avg F1=73.54 vs avg F1=45.12). This is accompanied with F1=60.04 on a Reddit dataset and F1=60.92 on an external evaluation set. Further analysis shows that only 36 posts is required for a stable bot classification. Investigation shows that bot post features have changed across the years and can be difficult to differentiate from human features, making bot detection a difficult and ongoing problem.

==> tables/expertweights.tex <==
\begin{table}[!htbp]
\centering
\begin{tabular}{|p{2cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
\hline
\textbf{Expert} & \textbf{BotBuster-1} & \textbf{BotBuster-2} & \textbf{BotBuster-3} & \textbf{BotBuster-4} \\ \hline
Username & 13.88 & 15.36 & 27.46 & 20.99 \\
Screenname & 10.43 & 15.41 & 20.57 & 20.89 \\ 
Description & 26.85 & 23.64 & 20.71 & 24.13 \\ 
User Metadata & 9.29 & 14.96 & 15.58 & 19.26 \\
Post \newline (account-level) & 40.46 & 30.63 & - & - \\
Post \newline (post-level) & - & - & 15.67 & 15.71 \\
\hline
\end{tabular}
\caption{Sampling of expert weights (\%) for each BotBuster variation for accounts with all information. A higher value reflects higher importance is placed on the expert.}
\label{tab:expertweights}
\end{table}

\begin{table}[!htbp]
\centering
\begin{tabular}{|p{1.6cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
\hline
\textbf{Expert} & \textbf{BotBuster-4.1} & \textbf{BotBuster-4.2} & \textbf{BotBuster-4.3} & \textbf{BotBuster-4.4} & \textbf{BotBuster-4.5} \\ \hline
Username &  - & 24.90 & 36.09 & 18.45 & 39.26 \\
Screenname & 31.46 & - & 21.02 & 20.85 & 21.13 \\
Description & 35.17 & 31.51 & 25.80 & - & 20.34 \\
User \newline metadata &  12.61 & 14.43 & - & 27.25 & 19.21 \\
Post \newline (account-level) & - & - & - & - & - \\
Post \newline (post-level) & 18.76 & 29.17 & 17.08 & 33.45 & - \\
\hline
\end{tabular}
\caption{Sampling of expert weights for best-performing BotBuster-4 variation with missing information.}
\label{tab:expertweights-4}
\end{table}

==> tables/expertweights2.tex <==
\begin{table*}[!htbp]
\centering
\begin{tabular}{|l|llllll|}
\hline
\textbf{Model} & \textbf{User name} & \textbf{Screen name} & \textbf{Description} & \textbf{User Metadata} & \textbf{Post (account-level)} & \textbf{Post (post-level)} \\ \hline
\multicolumn{7}{|l|}{\textbf{BotBuster variation for accounts with all information}} \\ 
BotBuster-1 &  13.88 & 10.43 & 26.85 & 9.29 & 40.46 & - \\
BotBuster-2 & 15.36 & 15.41 & 23.64 & 14.96 & 30.63 & - \\ 
BotBuster-3 & 27.46 & 20.57 & 20.71 & 15.58 & - & 15.67 \\ 
BotBuster-4 & 20.99 & 20.89 & 24.13 & 19.26 & - & 15.71 \\ \hline
\multicolumn{7}{|l|}{\textbf{BotBuster-4 variation for accounts with missing information}} \\ 
BotBuster 4.1 & - & 31.46 & 35.17 & 12.61 & - & 18.76 \\ 
BotBuster 4.2 & 24.90 & - & 31.51 & 14.43 & - & 29.17 \\ 
BotBuster 4.3 & 36.09 & 21.02 & 25.80 & - & - & 17.08 \\ 
BotBuster 4.4 & 18.45 & 20.85 & - & 27.25 & - & 33.45 \\ 
BotBuster 4.5 & 39.26 & 21.13 & 20.34 & - & - \\
\hline
\end{tabular}
\caption{Sampling of expert weights (\%) for each BotBuster variation for accounts with all information and the variations for BotBuster-4. A higher value reflects higher importance is placed on the expert.}
\label{tab:expertweights2}
\end{table*}

==> tables/indivexperts.tex <==
\begin{table}[!htbp]
\centering
\begin{tabular}{|l|l|}
\hline
\textbf{Expert} & \textbf{F1 score} \\ \hline
Username & 62.01 \\
Screenname & 62.01 \\
Description & 69.33 \\ 
User metadata & 62.38 \\ 
Posts (account-level) & 64.22 \\ 
Posts (account-level) + derived values & 72.98 \\
Posts (post-level) & 64.79 \\
Posts (post-level) + derived values & 74.50 \\ 
\hline
\end{tabular}
\caption{F1 accuracy scores of each experts}
\label{tab:indivexperts}
\end{table}

==> tables/individualexpertswclassical.tex <==
\begin{table}[!htbp]
\centering
\begin{tabular}{|p{4cm}p{3cm}|}
\hline
\textbf{Expert} & \textbf{Macro F1 score} \\ \hline
\multicolumn{2}{|l|}{\textbf{User name}} \\ 
Decision tree &  54.96\\ 
Support Vector Classifier & 54.96\\ 
Random Forest & 54.96 \\ 
BotBuster-formulation & 62.01 \\
\hline
\multicolumn{2}{|l|}{\textbf{Screen name}} \\ 
Decision tree & 59.70 \\ 
Support Vector Classifier & 60.79\\ 
Random Forest &  59.56\\ 
BotBuster-formulation & 62.01 \\
\hline
\multicolumn{2}{|l|}{\textbf{Description}} \\ 
Decision tree & 63.19 \\ 
Support Vector Classifier & 60.79\\ 
Random Forest & 60.79 \\ 
BotBuster-formulation & 69.33 \\
\hline
\multicolumn{2}{|l|}{\textbf{User metadata}} \\ 
Decision tree & 44.52 \\ 
Support Vector Classifier & 55.63 \\ 
Random Forest & 55.63 \\ 
BotBuster-formulation & 62.38 \\
\hline
\multicolumn{2}{|l|}{\textbf{Posts (account-level)}} \\
Decision tree & 61.48 \\ 
Support Vector Classifier & 59.34 \\ 
Random Forest & 59.34 \\ 
BotBuster-formulation & 64.22 \\ 
\hline
\multicolumn{2}{|l|}{\textbf{Posts (post-level)}} \\
Decision tree &  59.22 \\ 
Support Vector Classifier &  63.59\\ 
Random Forest &  63.32\\ 
BotBuster-formulation & 64.79 \\ 
\hline
\multicolumn{2}{|l|}{\textbf{Posts (post-level) + derived values}} \\
Decision tree &  67.44\\ 
Support Vector Classifier &  71.25\\ 
Random Forest &  72.15\\ 
BotBuster-formulation & 74.50 \\ 
\hline
\multicolumn{2}{|l|}{\textbf{Posts (account-level) + derived values}} \\
Decision tree &  68.74\\ 
Support Vector Classifier & 68.65\\ 
Random Forest &  61.81\\ 
BotBuster-formulation & 72.98 \\ 
\hline
\end{tabular}
\caption{Macro F1 accuracy scores of individual experts}
\label{tab:indivexpertswclassical}
\end{table}
